Grounding Language to Entities and Dynamics for Generalization in Reinforcement Learning

We investigate the use of natural language to drive the generalization of control policies and introduce the new multi-task environment Messenger with free-form text manuals describing the environment dynamics. Unlike previous work, Messenger does not assume prior knowledge connecting text and state observations $-$ the control policy must simultaneously ground the game manual to entity symbols and dynamics in the environment. We develop a new model, EMMA (Entity Mapper with Multi-modal Attention) which uses an entity-conditioned attention module that allows for selective focus over relevant descriptions in the manual for each entity in the environment. EMMA is end-to-end differentiable and learns a latent grounding of entities and dynamics from text to observations using only environment rewards. EMMA achieves successful zero-shot generalization to unseen games with new dynamics, obtaining a 40% higher win rate compared to multiple baselines. However, win rate on the hardest stage of Messenger remains low (10%), demonstrating the need for additional work in this direction.

==> figures/joined_table.tex <==
% \usepackage{arydshln}
\begin{table*}[t!]
\centering
\caption{Win rates (\& stddev.) on training games over 3 seeds. % \textit{All} is overall win rate, \textit{MC}, \textit{SC} denote multi and single-combination respectively. %Standard deviation ($\pm$) is over 3 seeds.
}\label{tab:train_winrates}

\resizebox{\linewidth}{!}{
\begin{sc}
\begin{tabular}{c|cccc|cccc|cccc}
\toprule
 & S1-All & S1-MC & S1-SC & S1-Test & S2-All & S2-MC & S2-SC & S2-Test & S3-All & S3-MC & S3-SC & S3-Test \\ 
\midrule
gid & $89\pm 3.8$ & $90\pm 5.5$ & $89\pm 3.7$ & $18\pm 8.2$ & $3.6\pm 0.6$ & $3.4\pm 0.7$ & $3.9\pm 1.5$ & $15\pm 1.1$ & $-$ & $-$ & $-$ & $-$ \\
bos & $90\pm 7.2$ & $91\pm 6.5$ & $90\pm 6.8$ & $6.7\pm 2.8$ & $2.1\pm 0.5$ & $2.9\pm 1.4$ & $2.4\pm 0.6$ & $16\pm 1.4$ & $-$ & $-$ & $-$ & $-$ \\
bayes & $84\pm 1.3$ & $97\pm 0.9$ & $51\pm 1.6$ & $66\pm 1.5$ & $69\pm 1.1$ & $85\pm 0.9$ & $22\pm 4.8$ & $39\pm 3.8$ & $1.0\pm 0.2$ & $1.5\pm 0.6$ & $1.1\pm0.8$ & $3.2\pm 0.3$ \\
txtpi & $\bm{98\pm2.1}$ & $\bm{98\pm2.9}$ & $\bm{99\pm1.7}$ & $2.5\pm1.7$ & $94\pm3.5$ & $95\pm2.1$ & $94\pm4.0$ & $1.1\pm0.5$ & $4.1\pm1.3$ & $3.3\pm0.5$ & $3.4\pm0.7$ & $3.3\pm0.7$ \\
emma & $88\pm 2.3$ & $88\pm 2.4$ & $87\pm 1.6$ & $\bm{85\pm 1.4}$ & $\bm{95\pm0.4}$ & $\bm{96\pm0.2}$ & $\bm{95\pm0.5}$ & $\bm{79\pm 1.9}$ & $\bm{5.2\pm 0.6}$ & $\bm{5.0\pm 0.8}$ & $\bm{4.9\pm0.2}$ & $\bm{5.6\pm 2.4}$ \\ 
\hdashline
oracle & $97\pm 0.8$ & $97\pm 0.3$ & $96\pm0.6$ & $97\pm 0.3$ & $96\pm 0.8$ & $96\pm 0.4$ & $94\pm 0.4$ & $82\pm 1.7$ & $93\pm 1.1$ & $92\pm 0.3$ & $92\pm1.0$ & $88\pm 1.0$ \\
\bottomrule
\end{tabular}
\end{sc}
}
\end{table*}
